Challenges in Designing Exploit Mitigations for Deeply Embedded Systems

Memory corruption vulnerabilities have been around for decades and rank among the most prevalent vulnerabilities in embedded systems. Yet this constrained environment poses unique design and implementation challenges that significantly complicate the adoption of common hardening techniques. Combined with the irregular and involved nature of embedded patch management, this results in prolonged vulnerability exposure windows and vulnerabilities that are relatively easy to exploit. Considering the sensitive and critical nature of many embedded systems, this situation merits significant improvement. In this work, we present the first quantitative study of exploit mitigation adoption in 42 embedded operating systems, showing the embedded world to significantly lag behind the general-purpose world. To improve the security of deeply embedded systems, we subsequently present {\mu}Armor, an approach to address some of the key gaps identified in our quantitative analysis. {\mu}Armor raises the bar for exploitation of embedded memory corruption vulnerabilities, while being adoptable on the short term without incurring prohibitive extra performance or storage costs.

==> app.tex <==
\appendix



\newpage

\setcounter{table}{0}




































































\section{Appendix: Detailed Quantitative Analysis Results}\label{apendix}
	
\begin{table}[!htbp]
	\tiny
	\centering
	\caption{Detailed Embedded OS exploit mitigation adoption. Red for Mobile embedded OSes, white for regular embedded OSes and gray for deeply embedded OSes.}
	\begin{tabular}{m{1.3cm}K{0.24cm}K{0.42cm}K{0.29cm}m{1.65cm}K{0.24cm}K{0.42cm}K{0.29cm}}
		\textbf{OS} & \textbf{ESP} & \textbf{ASLR} & \textbf{Can.} & \textbf{OS} &\textbf{ESP} & \textbf{ASLR} & \textbf{Can.}\\
		\hline	
		\rowcolor{LRed}	BlackBerry OS & \checkmark & \checkmark & \checkmark& Android\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{LRed} iOS\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & Win 10 Mob.\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{LRed} Sailfish OS\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & Tizen\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{white} Ubuntu Core\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark &  Brillo\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{white}Yocto Linux\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & Windows Embedded\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{white} OpenWRT\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & Junos OS\textsuperscript{$\ast$} & \checkmark & $\times$ & \checkmark \\
		\rowcolor{white} $\mu$Clinux\textsuperscript{$\ast$} & \checkmark & $\times$ & \checkmark & CentOS\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{white} NetBSD\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & IntervalZero RTX\textsuperscript{$\ast$} & \checkmark & $\times$ & \checkmark \\
		\rowcolor{white} ScreenOS & $\times$ & $\times$ & $\times$ & Enea OSE & $\times$ & $\times$ & $\times$ \\
		\rowcolor{white} QNX & \checkmark & \checkmark & \checkmark & VxWorks & \checkmark & $\times$ & $\times$ \\
		\rowcolor{white} INTEGRITY & \checkmark & $\times$ & $\times$ & \redactedOS \textsuperscript{2} & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} Cisco IOS & $\times$ & $\times$ & $\times$ & eCos & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} Zephyr & \checkmark & $\times$ & \checkmark & ThreadX & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} Nucleus & $\times$ & $\times$ & $\times$ & NXP MQX & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} Kadak AMX & $\times$ & $\times$ & $\times$ & Keil RTX & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} RTEMS & $\times$ & $\times$ & $\times$ & freeRTOS & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} Micrium $\mu$C/OS\textsuperscript{1} & \checkmark & $\times$ & $\times$ & TI-RTOS & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} DSP/BIOS & $\times$ & $\times$ & $\times$ & TinyOS & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} LiteOS & $\times$ & $\times$ & $\times$ & RIOT & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} ARM mbed & \checkmark & $\times$ & $\times$ & Contiki & $\times$ & $\times$ & $\times$ \\
		\rowcolor{gray!50} Nano-RK & $\times$ & $\times$ & $\times$ & Mantis & $\times$ & $\times$ & $\times$ \\
	\end{tabular}
	
	\label{table:os_mitigation_adoption}   
	\small \textsuperscript{ $\ast$} \emph{Embedded OS based on Windows, Linux or BSD.}\\
	\small \textsuperscript{1} \emph{A $\mu$C/OS-II kernel version with ESP support is available via a Micrium partner}\\
	\small \textsuperscript{2} Due to the sensitive nature of \redactedOS, we have received it on the condition of anonymity for the vendor. \redactedOS is a real-time OS which is primarily being used for aerospace applications.  




\bigskip



		\tiny
	\centering	
	\caption{Detailed Embedded OS exploit mitigation dependency support for Memory Protection (MPROT), Virtual Memory (VMEM) and Random Number Generator (RNG). Red  for Mobile embedded OSes, white for regular embedded OSes and gray for deeply embedded OSes.}
	\begin{tabular}{m{1cm}K{0.5cm}K{0.4cm}K{0.3cm}m{1cm}K{0.6cm}K{0.5cm}K{0.3cm}}
		\textbf{OS} & \textbf{MPROT} & \textbf{VMEM} & \textbf{RNG} & \textbf{OS} & \textbf{MPROT} & \textbf{VMEM} & \textbf{RNG}\\
		\hline
		\rowcolor{LRed}	Android\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & iOS\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{LRed}	Win10 Mob.\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & BlackBerry OS & \checkmark & \checkmark & \checkmark \\
		\rowcolor{LRed}	Tizen\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & Sailfish OS\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{white} Ubuntu Core\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & Brillo\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{white} Yocto Linux\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & Windows Embedded\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark\\
		\rowcolor{white} OpenWRT\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & Junos OS\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark\\
		\rowcolor{white} $\mu$Clinux\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & CentOS\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark \\
		\rowcolor{white} NetBSD\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark & IntervalZero RTX\textsuperscript{$\ast$} & \checkmark & \checkmark & \checkmark\\
		\rowcolor{white} ScreenOS & \checkmark & \checkmark & \checkmark & Enea OSE & \checkmark & \checkmark & $\times$\\
		\rowcolor{white} QNX & \checkmark & \checkmark & \checkmark & VxWorks & \checkmark & \checkmark & $\times$\\
		\rowcolor{white} INTEGRITY & \checkmark & \checkmark & \checkmark & \redactedOS & \checkmark & \checkmark & \checkmark\\
		\rowcolor{gray!50} Cisco IOS & $\times$ & $\times$ & \checkmark & eCos & $\times$ & $\times$ & $\times$\\
		\rowcolor{gray!50} Zephyr& \checkmark & $\times$ & $\times$ & ThreadX & \checkmark & $\times$ & $\times$\\
		\rowcolor{gray!50} Nucleus & \checkmark & $\times$ & $\times$ & NXP MQX & \checkmark & $\times$ & $\times$\\
		\rowcolor{gray!50} Kadak AMX & $\times$ & $\times$ & $\times$ & Keil RTX & \checkmark & $\times$ & $\times$\\
		\rowcolor{gray!50} RTEMS & $\times$ & $\times$ & $\times$ & FreeRTOS & \checkmark & $\times$ & $\times$\\
		\rowcolor{gray!50} Micrium $\mu$C/OS & \checkmark & $\times$ & $\times$ & TI-RTOS & \checkmark & $\times$ & $\times$\\
		\rowcolor{gray!50} DSP/BIOS & \checkmark & $\times$ & $\times$ & TinyOS & \checkmark & $\times$ & $\times$\\
		\rowcolor{gray!50} LiteOS & \checkmark & $\times$ & $\times$ & RIOT & \checkmark & $\times$ & $\times$\\
		\rowcolor{gray!50} ARM mbed & \checkmark & $\times$ & $\times$ & Contiki & $\times$ & $\times$ & $\times$\\
		\rowcolor{gray!50} Nano-RK & $\times$ & $\times$ & $\times$ & Mantis & $\times$ & $\times$ & $\times$\\
	\end{tabular}
	
	\label{table:os_feature_support}   
	\small \textsuperscript{ $\ast$} \emph{Embedded OS based on Windows, Linux or BSD.}\\

\end{table}






\begin{table}[!htbp]
\scriptsize
	\centering
	\caption{Core Family dependency support in Harvard (H) and Von Neumann (N) architectures. We consider a feature supported if it is supported by all members of a given core family and absent if it is not supported by any of them. Any variation with regards to dependency support is denoted with $\sim$ and omitted from aggregated results.}
	\begin{tabular}{lcccc}
		\textbf{Core Family} & \textbf{Arch.} & \textbf{MPU} & \textbf{MMU} & \textbf{ESP} \\
		\hline
		\textbf{ARM} & & & & \\
		\hdashline
		ARM1 & N & $\times$ & $\times$ & $\times$ \\
		ARM2 & N & $\times$ & $\times$ & $\times$ \\
		ARM3 & N & $\times$ & $\times$ & $\times$ \\
		ARM6 & N & $\times$ & $\times$ & $\times$ \\
		ARM7 & N & $\times$ & $\times$ & $\times$ \\
		ARM7T & N & $\sim$ & $\sim$ & $\times$ \\
		ARM7EJ & N & $\times$ & $\times$ & $\times$ \\
		ARM8 & N & $\times$ & \checkmark & $\times$ \\
		ARM9T & N & $\sim$ & $\sim$ & $\times$ \\
		ARM9E & N & $\sim$ & $\sim$ & $\times$ \\
		ARM10E & N & $\times$ & \checkmark & $\times$ \\
		ARM11 & N & $\sim$ & $\sim$ & \checkmark \\
		ARM Cortex-A & N & $\times$ & \checkmark & \checkmark \\
		ARM Cortex-R & N & \checkmark & $\times$ & \checkmark \\
		ARM Cortex-M & N & $\sim$ & $\times$ & \checkmark \\
		\hline
		\textbf{PIC} & & & & \\
		\hdashline
		PIC10 & H & $\times$ & $\times$ & $\times$ \\
		PIC12 & H & $\times$ & $\times$ & $\times$ \\
		PIC16 & H & $\times$ & $\times$ & $\times$ \\
		PIC18 & H & $\times$ & $\times$ & $\times$ \\
		PIC24 & H & $\times$ & $\times$ & $\times$ \\
		dsPIC & H & $\times$ & $\times$ & $\times$ \\
		\hline
		\textbf{MIPS32} & & & & \\
		\hdashline
		PIC32MX & N & $\times$ & $\times$ & $\times$ \\
		PIC32MZ EC & N & $\times$ & \checkmark & $\times$ \\
		PIC32MZ EF & N & $\times$ & \checkmark & \checkmark \\
		PIC32MM & N & $\times$ & \checkmark & \checkmark \\
		\hline
		\textbf{PowerPC} & & & & \\
		\hdashline
		PPC e200 & N & $\sim$ & $\sim$ & \checkmark \\
		PPC e300 & N & $\times$ & \checkmark & \checkmark \\
		PPC e500 & N & $\times$ & \checkmark & \checkmark \\
		PPC e600 & N & $\times$ & \checkmark & \checkmark \\
		PPC 403 & N & $\times$ & $\times$ & $\times$ \\
		PPC 401 & N & $\times$ & $\times$ & $\times$ \\
		PPC 405 & N & $\times$ & \checkmark & \checkmark \\
		PPC 440 & N & $\times$ & \checkmark & \checkmark \\
		PPC 740 & N & $\times$ & \checkmark & \checkmark \\
		PPC 750 & N & $\times$ & \checkmark & \checkmark \\
		PPC 603 & N & $\times$ & \checkmark & \checkmark \\
		PPC 604 & N & $\times$ & \checkmark & \checkmark \\
		PPC 7400 & N & $\times$ & \checkmark & \checkmark \\
	\end{tabular}
	\label{table:hardware_feature_support_a}
\end{table}









\begin{table}[!htbp]
	\scriptsize
	\centering
	\caption{Core Family dependency support in Harvard (H) and Von Neumann (N) architectures II}
	\begin{tabular}{lcccc}
		\textbf{Core Family} & \textbf{Arch.} & \textbf{MPU} & \textbf{MMU} & \textbf{ESP} \\
		\hline
		\textbf{x86} & & & & \\
		\hdashline
		Intel Atom Z34XX & N & $\times$ & \checkmark & \checkmark \\
		Intel Quark X10XX & N & $\times$ & \checkmark & \checkmark \\
		Intel Quark $\mu$C\textsuperscript{1} & N & $\times$ & \checkmark & \checkmark \\
		\hline
		\textbf{SuperH} & & & & \\
		\hdashline
		SH-1 & N & $\times$ & $\times$ & $\times$ \\
		SH-2 & N & $\times$ & $\times$ & $\times$ \\
		SH-3 & N & $\times$ & \checkmark & $\times$ \\
		SH-4 & N & $\times$ & \checkmark & $\times$ \\
		\hline
		\textbf{AVR} & & & & \\
		\hdashline
		ATtiny & H & $\times$ & $\times$ & $\times$ \\
		ATmega & H & $\times$ & $\times$ & $\times$ \\
		ATxmega & H & $\times$ & $\times$ & $\times$ \\
		\hline
		\textbf{AVR32} & & & & \\
		\hdashline
		AVR32A & N & \checkmark & $\times$ & $\times$ \\
		AVR32B & N & $\times$ & \checkmark & $\times$ \\
		\hline
		\textbf{8051} & & & & \\
		\hdashline
		Intel MCS-51 & H & $\times$ & $\times$ & $\times$ \\
		Infineon XC88X-I & H & $\times$ & $\times$ & $\times$ \\
		Infineon XC88X-A & H & $\times$ & $\times$ & $\times$ \\
		\hline
		\textbf{m68k} & & & & \\
		\hdashline
		NXP M683XX & N & $\times$ & $\times$ & $\times$ \\
		NXP ColdFire V1 & N & $\times$ & $\times$ & $\times$ \\
		NXP ColdFire V2 & N & $\times$ & $\times$ & $\times$ \\
		NXP ColdFire V3 & N & $\times$ & $\times$ & $\times$ \\
		NXP ColdFire V4 & N & $\times$ & \checkmark & $\times$ \\
		NXP ColdFire V5 & N & $\times$ & \checkmark & $\times$ \\
		\hline
		\textbf{TriCore} & & & & \\
		\hdashline
		Infineon TC11xx & H & $\times$ & $\sim$ & $\times$ \\
		Infineon AUDO Future & H & $\times$ & $\times$ & $\times$ \\
		\hline
		\textbf{C166} & & & & \\
		\hdashline
		Infineon XE166 & N & \checkmark & $\times$ & \checkmark \\
		Infineon XC2200 & N & \checkmark & $\times$ & \checkmark \\
		\hline
		\textbf{MSP430} & & & & \\
		\hdashline
		MSP430x1xx & N & $\times$ & $\times$ & $\times$ \\
		MSP430x2xx & N & $\times$ & $\times$ & $\times$ \\
		MSP430x3xx & N & $\times$ & $\times$ & $\times$ \\
		MSP430x4xx & N & $\times$ & $\times$ & $\times$ \\
		MSP430x5xx & N & $\times$ & $\times$ & $\times$ \\
		MSP430x6xx & N & $\times$ & $\times$ & $\times$ \\
		MSP430FRxx & N & \checkmark & $\times$ & $\times$ \\
		\hline
		\textbf{Blackfin} & & & & \\
		\hdashline
		Analog Blackfin\textsuperscript{2} & N & \checkmark & $\times$ & $\times$ \\
		\hline
		\textbf{ARC} & & & & \\
		\hdashline
		Synopsys ARC EM & H & $\sim$ & $\times$ & $\times$ \\
		Synopsys ARC 600 & H & $\sim$ & $\times$ & $\times$ \\
		Synopsys ARC 700 & H& $\times$ & $\sim$ & $\times$ \\
		\hline
		\textbf{RL78} & & & & \\
		\hdashline
		Renesas RL78/G1x & H & $\times$ & $\times$ & $\times$ \\
		Renesas RL78/L1x & H & $\times$ & $\times$ & $\times$ \\
		\hline
		\textbf{RX} & & & & \\
		\hdashline
		Renesas RX200 & H & $\sim$ & $\times$ & $\times$ \\
		Renesas RX600 & H & $\sim$ & $\times$ & $\times$ \\		
	\end{tabular}
	
	
	\label{table:hardware_feature_support_b}
	\small \textsuperscript{1} \emph{Intel Quark Microcontrollers (D1000/C1000/D2000)}\\
	\small \textsuperscript{2} \emph{Although documentation mentions an MMU, it does not support address translation (and thus does not allow for virtual memory) which is why we consider it an MPU for our purposes}
\end{table}










\begin{table}[!htbp]
	\scriptsize
	\centering
	\caption{\uScramble Coverage Analysis.}
	\begin{tabular}{p{1.15cm}K{0.8cm}K{0.8cm}|p{1.0cm}K{0.8cm}K{0.8cm}}
		\textbf{Set} & \textbf{Avg. GS\textsuperscript{1}} & \textbf{Max. GS\textsuperscript{1}} & \textbf{Set} & \textbf{Avg. GS\textsuperscript{1}} & \textbf{Max. GS\textsuperscript{1}} \\
		\hline
		\textbf{Application} & & & \textbf{Application} & & \\
		\hdashline
		\texttt{lift} & 2 & 9 &	\texttt{cover} & 29.8 & 143 \\ 
		\texttt{powerwindow} & 1.2 & 10 & \texttt{duff} & 1.6 & 7 \\
		&&&\texttt{test3} & 0 & 0 \\
		\hline
		\textbf{Kernel} & & &\textbf{Sequential} & &  \\
		\hdashline
		\texttt{binarysearch} & 1.4 & 13 & \texttt{adpcm\_dec} & 0.5 & 4 \\
		\texttt{bitcount} & 63.3 & 180 & 	\texttt{adpcm\_enc} & 0.6 & 5 \\
		\texttt{bitonic} & 85.15 & 166 & \texttt{ammunition} & 3.6 & 147 \\
		\texttt{bsort} & 58.5 & 171 & \texttt{anagram} & 0.6 & 4 \\
		\texttt{complex\_updates} & 68.1 & 199 &	\texttt{audiobeam} & 4 & 79 \\
		\texttt{countnegative} & 2 & 11 & \texttt{cjpeg\_transupp} & 32 & 96 \\
		\texttt{fac} & 2.5 & 4 &\texttt{cjpeg\_wrbmp} & 1.4 & 3 \\
		\texttt{fft} & 1.2 & 5 & 	\texttt{dijkstra} & 1.3 & 5 \\
		\texttt{filterbank} & 59.9 & 209 &	\texttt{epic} & 0 & 0 \\
		\texttt{fir2dim} & 70.5 & 210 & 	\texttt{fmref} & 0.5 & 3 \\
		\texttt{iir} & 2.5 & 8 & \texttt{gsm\_dec} & 1.3 & 43 \\
		\texttt{insertsort} & 101.5 & 202 	& \texttt{h264\_dec} & 100 & 181 \\
		\texttt{jfdctint} & 97 & 193 & 	\texttt{huff\_dec} & 18.8 & 91 \\
		\texttt{lms} & 64.2 & 193 & 	\texttt{huff\_enc} & 5.8 & 55 \\
		\texttt{ludcmp} & 55.4 & 166 & 	\texttt{mpeg2} & 0 & 0 \\
		\texttt{matrix1} & 68.8 & 203 &	\texttt{ndes} & 0.6 & 2 \\
		\texttt{md5} & 0.6 & 7 & 	\texttt{petrinet} & 2 & 2 \\
		\texttt{minver} & 1.3 & 5 & 	\texttt{rijndael\_dec} & 2.5 & 16 \\
		\texttt{pm} & 12.5 & 97 &	\texttt{rijndael\_enc} & 3 & 11 \\
		\texttt{prime} & 0.9 & 5 & \texttt{statemate} & 16.4 & 97 \\
		\texttt{quicksort} & 1.5 & 9 &&&\\
		\texttt{recursion} & 91.6 & 188 &&&\\
		\texttt{sha} & 2.3 & 6 &&&\\
		\texttt{st} & 0.8 & 3 &&&\\
		\texttt{basicmath} & 1 & 4 &&&\\
		
		
	\end{tabular}
	
	\label{table:uscramble_coverage_analysis1}
	\small \textsuperscript{1} \emph{Gadget Survival}
\end{table}
\newpage
\section{Appendix: EPOXY Limitations}\label{epoxy}




There are several key limitations to the EPOXY~\cite{clements2017protecting} work that set it apart from \uArmor.

First, \uArmor targets a class of deeply embedded systems not addressed by EPOXY: those running an OS. EPOXY was designed to protect single-stack bare-metal embedded systems and is not suitable for deployment on multi-stack RTOS systems without significant re-engineering (e.g., such as with regards to scalability of safe-stack overhead, integrating privilege overlays transparently with OS mechanisms).




Secondly, EPOXY privilege overlay security model could be broken by an attacker returning to any legitimate call-site where the privilege elevation handler is invoked. Consider, for example, the Algorithm~\ref{algo}:\\


\begin{algorithm}
\caption{EPOXY Privilege Overlay Issue}\label{algo}
\begin{algorithmic}[1]
	
	\STATE Begin REQUEST PRIVILEGED EXECUTION
	\STATE Save Register and Flags State
	\IF {In Unprivileged Mode} 
	\STATE Execute SVC 0xFE (Elevate Privileges)
	\ENDIF
	\STATE Restore Register and Flags
	\STATE Execute Restricted Operation
	\STATE Set Bit 0 of Control Register (Reduces Privileges)
	\STATE END

\end{algorithmic}

\end{algorithm}

Here an attacker could return to line 2 where SVC 0xFE would invoke the custom EPOXY SVC\_Handler~\cite{epoxysrc}. The handler would check whether the interrupt source was correct regardless of unprivileged control-flow leading up to it and as such would elevate privileges allowing the attacker to execute the restricted operation in line 7. Code diversification would not help much because many restricted operations are located at static or easily obtainable addresses (e.g., extracted from the IVT).

Fourth, EPOXY code diversification approach is less fine-grained than that of \uArmor since it only randomizes function order but does not diversify function sizes (and thus leaves gadget offsets with respect to function addresses intact) nor does it reorder register preservation code. As such, EPOXY code diversification is more vulnerable to information leaks than \uArmor.

Finally, unlike \uArmor, EPOXY does not protect against ret2bootloader style attacks~\cite{francillonharvardinjection,zeronightsavr,goodspeed_sage_advice:2013} because it leaves sensitive bootloader code that cannot be relocated executable after system initialization As a result, an attacker can return to potentially sensitive code areas allowing for re-flashing code memory or disabling the MPU.















